Tempered stable distributions and finite variation Ornstein-Uhlenbeck processes

Constructing \Levy-driven Ornstein-Uhlenbeck processes is a task closely related to the notion of self-decomposability. In particular, their transition laws are linked to the properties of what will be hereafter called the \emph{a-reminder} of their self-decomposable stationary laws. In the present study we fully characterize the L\'evy triplet of these a-reminder s and we provide a general framework to deduce the transition laws of the finite variation Ornstein-Uhlenbeck processes associated with tempered stable distributions. We focus finally on the subclass of the exponentially-modulated tempered stable laws and we derive the algorithms for an exact generation of the skeleton of Ornstein-Uhlenbeck processes related to such distributions, with the further advantage of adopting a procedure computationally more efficient than those already available in the existing literature.

==> Tables/ptsou0_1_365.tex <==
\begin{table}[ht!]
    \centering\scriptsize
        \resizebox{\textwidth}{!}{
        \begin{tabular}{*{13}{|c|ccr|ccr|ccr|ccr}}
                    \hline
&       \multicolumn{3}{c|}{$c_{X, 1}(0,t)$} & \multicolumn{3}{c|}{$c_{X, 2}(0,t)$} & \multicolumn{3}{c|}{$c_{X, 3}(0,t)$} & \multicolumn{3}{c|}{$c_{X, 4}(0,t)$} \\
                    \hline
$p$ & true & MC & err \% & true & MC & err \% & true & MC & err \% & true & MC & err \% \\
\hline
$2.0$ & $0.0133$ & $0.0132$ & $1.4$ & $0.0083$ & $0.0081$ & $2.7$ & $0.00607$ & $0.00583$ & $4.0$ & $0.00503$ & $0.00496$ & $1.4$\\
$2.5$ & $0.0149$ & $0.0150$ & $-0.4$ & $0.0096$ & $0.0097$ & $-0.5$ & $0.00699$ & $0.00697$ & $0.3$ & $0.00558$ & $0.00545$ & $2.3$\\
$3.0$ & $0.0162$ & $0.0164$ & $-1.4$ & $0.0108$ & $0.0110$ & $-1.6$ & $0.00791$ & $0.00803$ & $-1.6$ & $0.00623$ & $0.00628$ & $-0.8$\\
$3.5$ & $0.0172$ & $0.0171$ & $0.5$ & $0.0118$ & $0.0118$ & $0.1$ & $0.00877$ & $0.00885$ & $-0.9$ & $0.00690$ & $0.00708$ & $-2.7$\\
                    \hline
        \end{tabular}
        }
    \scriptsize
    \caption{\footnotesize{Comparing the first four true cumulants
    with their corresponding estimated values obtained from $10^6$
simulations of $p\,$TS-OU processes with
$\alpha=0,\:t=\,\!^1/_{365}$ and $\left(b, c, \beta\right) =
\left(36, 0.4, 3\right)$}}\label{tab:ptsou0:1:365}
\end{table}


==> Tables/ptsou0_30_365.tex <==
\begin{table}[ht!]
    \centering\scriptsize
        \resizebox{\textwidth}{!}{
        \begin{tabular}{*{13}{|c|ccr|ccr|ccr|ccr}}
                    \hline
    &       \multicolumn{3}{c|}{$c_{X, 1}(0,t)$} & \multicolumn{3}{c|}{$c_{X, 2}(0,t)$} & \multicolumn{3}{c|}{$c_{X, 3}(0,t)$} & \multicolumn{3}{c|}{$c_{X, 4}(0,t)$} \\
                    \hline
$p$ & true & MC & err \% & true & MC & err \% & true & MC & err \% & true & MC & err \% \\
\hline
$2.0$ & $0.1348$ & $0.1345$ & $0.2$ & $0.0462$ & $0.0461$ & $0.2$ & $0.02368$ & $0.02369$ & $0.0$ & $0.01543$ & $0.01550$ & $-0.5$\\
$2.5$ & $0.1506$ & $0.1506$ & $0.0$ & $0.0536$ & $0.0535$ & $0.2$ & $0.02729$ & $0.02713$ & $0.6$ & $0.01712$ & $0.01692$ & $1.1$\\
$3.0$ & $0.1631$ & $0.1631$ & $0.0$ & $0.0601$ & $0.0601$ & $0.1$ & $0.03086$ & $0.03078$ & $0.3$ & $0.01911$ & $0.01903$ & $0.4$\\
$3.5$ & $0.1731$ & $0.1733$ & $-0.1$ & $0.0658$ & $0.0659$ & $-0.1$ & $0.03422$ & $0.03429$ & $-0.2$ & $0.02115$ & $0.02117$ & $-0.1$\\
                    \hline
        \end{tabular}
        }
    \scriptsize
    \caption{\footnotesize{Comparing the first four true cumulants
with their corresponding estimated values obtained from $10^6$
simulations of $p\,$TS-OU processes with
$\alpha=0,\;t=\,\!^{30}/_{365}$ and $\left(b, c, \beta\right) =
\left(36,0.4,3\right)$}}\label{tab:ptsou0:30:365}
\end{table}

